Star Cluster Classification using Deep Transfer Learning with PHANGS-HST

Currently available star cluster catalogues from HST imaging of nearby galaxies heavily rely on visual inspection and classification of candidate clusters. The time-consuming nature of this process has limited the production of reliable catalogues and thus also post-observation analysis. To address this problem, deep transfer learning has recently been used to create neural network models which accurately classify star cluster morphologies at production scale for nearby spiral galaxies (D < 20 Mpc). Here, we use HST UV-optical imaging of over 20,000 sources in 23 galaxies from the Physics at High Angular Resolution in Nearby GalaxieS (PHANGS) survey to train and evaluate two new sets of models: i) distance-dependent models, based on cluster candidates binned by galaxy distance (9-12 Mpc, 14-18 Mpc, 18-24 Mpc), and ii) distance-independent models, based on the combined sample of candidates from all galaxies. We find that the overall accuracy of both sets of models is comparable to previous automated star cluster classification studies (~60-80 per cent) and show improvement by a factor of two in classifying asymmetric and multi-peaked clusters from PHANGS-HST. Somewhat surprisingly, while we observe a weak negative correlation between model accuracy and galactic distance, we find that training separate models for the three distance bins does not significantly improve classification accuracy. We also evaluate model accuracy as a function of cluster properties such as brightness, colour, and SED-fit age. Based on the success of these experiments, our models will provide classifications for the full set of PHANGS-HST candidate clusters (N ~ 200,000) for public release.

==> affiliations.tex <==
\newcommand{\UCR}{\affil{Department of Physics $\And$ Astronomy, University of California, Riverside, CA, 92507, USA}}
\newcommand{\STSCI}{\affil{Space Telescope Science Institute, Baltimore, MD, 21218, USA}}
\newcommand{\Gemini}{\affil{Gemini Observatory/NSF’s NOIRLab, 950 N. Cherry Avenue, Tucson, AZ, 85719, USA}}
\newcommand{\Arizona}{\affil{Steward Observatory, University of Arizona, Tucson, AZ 85721, USA}}
\newcommand{\JHU}{\affil{Department of Physics and Astronomy, The Johns Hopkins University, Baltimore, MD 21218, USA}}
\newcommand{\TAPIR}{\affil{TAPIR, California Institute of Technology, Pasadena, CA 91125, USA}}
\newcommand{\Argonne}{\affil{Data Science and Learning Division, Argonne National Laboratory, Lemont, Illinois 60439, USA}}
\newcommand{\Chicago}{\affil{Department of Computer Science, University of Chicago, Chicago, Illinois 60637, USA}}
\newcommand{\Illinois}{\affil{Department of Physics, University of Illinois at Urbana-Champaign, Urbana, Illinois 61801, USA}}
\newcommand{\ITA}{\affil{Zentrum f{\"u}r Astronomie der Universit{\"a}t Heidelberg, Institut f{\"u}r Theoretische Astrophysik, D-69120 Heidelberg, Germany}}
\newcommand{\UHInter}{\affil{Universit{\"a}t Heidelberg, Interdiszipli{\"a}res Zentrum f{\"u}r Wissenschaftliches Rechnen, D-69120 Heidelberg, Germany}}
\newcommand{\CITEVA}{\affil{Centro de Astronom\'ia (CITEVA), Universidad de Antofagasta, Avenida Angamos 601, Antofagasta, Chile}}
\newcommand{\Wyoming}{\affil{Department of Physics \& Astronomy, University of Wyoming, Laramie, WY, 82071, USA}}
\newcommand{\COOL}{\affil{Cosmic Origins Of Life (COOL) Research DAO, coolresearch.io}}
\newcommand{\ANU}{\affil{Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT 2611, Australia; kathryn.grasha@anu.edu.au}}
\newcommand{\ARC}{\affil{ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), Australia}}
\newcommand{\UCM}{\affil{Departamento de Física de la Tierra y Astrof\'isica, UCM, 28040 Madrid, Spain}}
\newcommand{\MPIA}{\affil{Max Planck Institut f{\"u}r Astronomie, K{\"o}nigstuhl17, 69117 Heidelberg, Germany}}
\newcommand{\ARI}{\affil{Astronomisches Rechen-Institut, Zentrum f{\"u}r Astronomie der Universit{\"a}t Heidelberg, M{\"o}nchofstra{\ss}e 12-14, D-69120 Heidelberg, Germany}}
\newcommand{\UWA}{\affil{International Centre for Radio Astronomy Research, The University of Western Australia, 7 Fairway, Crawley, WA 6009, Australia}}
\newcommand{\Stromlo}{\affil{Research School of Astronomy and Astrophysics, Australian National University, Mt. Stromlo Observatory, Weston Creek, ACT 2611, Australia}}
\newcommand{\TUM}{\affil{Technical University of Munich, School of Engineering and Design, Department of Aerospace and Geodesy, Chair of Remote Sensing Technology, \\\hspace{2.2mm}Arcisstr. 21, 80333 Munich, Germany}}
\newcommand{\Stockholm}{\affil{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}}


\hyphenation{Cosmic-Flows}
\hyphenation{Hyper-LEDA}
\hyphenation{HERA-CLES}

==> authors.tex <==
\begin{document}
\correspondingauthor{Stephen Hannon}
\email{hannon@mpia.de}

\author[0000-0001-6038-9511]{Stephen Hannon}
\UCR
\MPIA

\author[0000-0001-6038-9511]{Bradley C. Whitmore}
\STSCI

\author[0000-0001-6038-9511]{Janice C. Lee}
\Gemini
\Arizona
\STSCI

\author[0000-0001-6038-9511]{David A. Thilker}
\JHU

\author[0000-0001-6038-9511]{Sinan Deger}
\TAPIR
\Stockholm

\author[0000-0001-6038-9511]{E.~A. Huerta}
\Argonne
\Chicago
\Illinois

\author[0000-0001-6038-9511]{Wei Wei}
\Illinois

\author[0000-0001-6038-9511]{Bahram Mobasher}
\UCR

\author[0000-0001-6038-9511]{Ralf Klessen}
\ITA
\UHInter

\author[0000-0001-6038-9511]{M\'ed\'eric Boquien}
\CITEVA

\author[0000-0001-6038-9511]{Daniel~A.~Dale}
\Wyoming

\author[0000-0001-6038-9511]{M\'elanie Chevance}
\ITA
\COOL

\author[0000-0001-6038-9511]{Kathryn Grasha}
\ANU
\ARC

\author[0000-0001-6038-9511]{Patricia Sanchez-Blazquez}
\UCM

\author[0000-0001-6038-9511]{Thomas Williams}
\MPIA

\author[0000-0001-6038-9511]{Fabian Scheuermann}
\ARI

\author[0000-0001-6038-9511]{Brent Groves}
\UWA
\Stromlo

\author[0000-0001-6038-9511]{Hwihyun Kim}
\Gemini

\author[0000-0001-6038-9511]{J.~M.~Diederik Kruijssen}
\COOL
\TUM

\author{the PHANGS-HST Team}


